What Do We See: An Investigation Into the Representation of Disability in Video Games

There has been a large body of research focused on the representation of gender in video games. Disproportionately, there has been very little research in respect to the representation of disability. This research was aimed at examining the representation of disabled characters through a method of content analysis of trailers combined with a survey of video gamers. The overall results showed that disabled characters were under-represented in videogames trailers, and respondents to the survey viewed disabled characters as the least represented group. Both methods of research concluded that the representation of disabled characters was low. Additionally, the characters represented were predominantly secondary, non-playable characters not primary. However, the research found that the defined character type was a mixture of protagonists and antagonists, bucking the standard view of disabled characters in video games.

==> TitlePage.tex <==
\begin{titlepage}
\begin{center}
\vspace*{1cm}

\textbf{ \large{What Do We See: An Investigation Into the Representation of Disability in Video Games}}

\vspace{1.5cm}

% Author names and affiliations
Dr. Jethro Shell$^{a}$ (jethros@dmu.ac.uk)\\

\hspace{10pt}

\begin{flushleft}
\small  
$^a$ Institute of Artificial Intelligence, De Montfort University, The Gateway, Leicester, LE1 9BH, United Kingdom  \\

\vspace{1cm}
\textbf{Corresponding Author:} \\
Dr. Jethro Shell \\
Institute of Artificial Intelligence, De Montfort University, The Gateway, Leicester, LE1 9BH, United Kingdom  \\
Tel: +44(0)116 2078520\\
Email: jethros@dmu.ac.uk

\end{flushleft}        
\end{center}
\end{titlepage}
